SuperB Technical Design Report

In this Technical Design Report (TDR) we describe the SuperB detector that was to be installed on the SuperB e+e- high luminosity collider. The SuperB asymmetric collider, which was to be constructed on the Tor Vergata campus near the INFN Frascati National Laboratory, was designed to operate both at the Upsilon(4S) center-of-mass energy with a luminosity of 10^{36} cm^{-2}s^{-1} and at the tau/charm production threshold with a luminosity of 10^{35} cm^{-2}s^{-1}. This high luminosity, producing a data sample about a factor 100 larger than present B Factories, would allow investigation of new physics effects in rare decays, CP Violation and Lepton Flavour Violation. This document details the detector design presented in the Conceptual Design Report (CDR) in 2007. The R&D and engineering studies performed to arrive at the full detector design are described, and an updated cost estimate is presented. A combination of a more realistic cost estimates and the unavailability of funds due of the global economic climate led to a formal cancelation of the project on Nov 27, 2012.

==> DCH/DCH_RandD.tex <==
\tdrsec{R\&D Program - {\color{green} Finocchiaro, Piccolo} {\color{red} 6 pages}}
\label{sec:DCH_RandD}
The \babar\ DCH operational record has been quite good, both for what performances and
reliability is concerned; however there are possible paths of improvements that one would
like to explore, so that the \superb\ DCH performances could be yet better that the \babar\ one.
In particular, advances in front-end and DAQ electroncs might grant the possibility to implement 
the {\it cluster counting} technique, that in principle hold the promise of a much better \dEdx
resolution and of a substantial improvement on spatial performances.
In order to asses both the feasibility and the operational improvements for the {\it cluster 
counting} technique  a complete R\& D program has been proposed: the latter includes both beam
test and cosmic ray stands to monitor performancs of {\it ad hoc} built prototypes. 
While the \dEdx resolution gain of the cluster counting method is in principle quite sizeable
compared to the traditional total charge collection, the former in fact  does not present Landau 
fluctuation, the actual capability of the {\bf measured} number of cluster might not retain 
the same analyzing power, due to a pletora of experimental effects that should be studied in 
details so that  the energy loss measurement  derating  should be assessed and, if
possible, cured.
A (partial) lists of effects that need study is:
\begin{itemize}
\item  Algorithmic capability to detect clusters 
\item Electronics and environmental noise
\item Geeometrical effects
\item Dispersive effects on pulses travelling on the wires
\item Optimal electronics bandwidth
\item Optimization of  gas miscture
\item Required stability for gas mixture
\end{itemize}
Few prototypes were built and operated to answer the above mentioned questions.
The first one (Proto 1), a small chamber, 30 cm. long,  with a gell geometry resembling  the 
the original \babar\ chamber (including about 30 cells), was used to study drift properties of
different gas mixtures; no attempt was made to eveluate how cluster counting could be implemented.
The main information that was extracted from  Proto 1 concerned total drift time and spatial 
resolution attainable with
different gas mixture as compared to what \babar\ DCH  had been able to deliver.
%Non so se vale la pena di mettere un paio di figure%
Two more Prototypes were build: Proto 2, a full length (2.5 m.) prototype with the same 
(rectangular) cell geometry proposted for the SupeB DCH, including 28 cells, and a single cell 
prototype SW1, again full length. 
Both Proto 2 and SW1 are at the moment operational and collecting data on cosimc ray stands; both
devices have been exposed to test beams, a 500 MeV/c electron beam Proto 2, a variety of pion 
and/or Kaon beams at various momenta SW1.
Few construction details for Proto 2: the wire structure that mimics a small part of proposed
\superb\ DCH is surrounded by guard wires to obtain a well behaved field distribution at the 
boundary of the active detector volume. There are few construction differences between cells 
so that alternate  technical solutions could be tested: few cells have a traditional W sense 
wires, the majority of cells however have  a Molybdenum sense wire. Even if Molybdenum has 
mechanical properties not as good as Tungsten, its electrical properties, {\it e.g.} its 
resistance, is lower than the latter. This, in turn, will imply smaller dispersion for pulses 
travelling  along the wires.
The entire wire structure is enclosed in an Aluminum container 5 mm thick: three thin windows
have been carved in the middle and at the extremities in order to have smaller amount of 
material in the path of low energy particles measured by this device.

  
 

\tdrsubsec{Results}
\tdrsubsec{Plans}



==> ELEX/ELEX-CablePlant.tex <==
\tdrsubsec{Cable Plant}

{\color{blue} This section has been incorporated in the Power Supply section}


==> ELEX/ELEX-Grounding.tex <==
\tdrsubsec{Grounding and Shielding}

{\color{blue} This section has been incorporated in the Power Supply section}



==> EMC/EMC-BWD-BtoTauNu.tex <==
\subsection{$B \rightarrow \tau \nu$}

The study of the leptonic decay $B \rightarrow \tau \nu$ is of particular interest as a test 
of the Standard Model (SM) and a probe for New Physics. The presence of a charged Higgs boson 
(in {\it e.g.}, a Two Higgs Doublet Model) as a decay mediator could significantly enhance 
the branching ratio above the SM value. A detailed analysis of this channel is therefore 
quite important in searches for physics beyond the SM.

The $B \rightarrow \tau \nu$ decay is challenging to identify, as the final state contains many 
neutrinos and can only be partially reconstructed. Signal events are selected using a recoil 
analysis, where the signal $B$-meson is identified as the recoiling system against 
the other (tag) $B$ meson. The tag $B$-meson is either fully reconstructed via its hadronic 
decays~\cite{?}, or partially reconstructed from its semileptonic 
$B \rightarrow D^0 \mu \nu_\mu, D^0 \rightarrow K\pi$ decays. The rest of the event is assigned to the 
$B \rightarrow \tau \nu$ candidate, and must be compatible with one of the following decay modes 
of the tau lepton: 
$\mu\nu_\mu\nu_\tau$, $e\nu_e\nu_\tau$, $\pi\nu_\tau$, $\pi\pi^0\nu_\tau$, 
$\pi\pi^0\pi^0\nu_\tau$, $\pi\pi\pi\nu_\tau$, $\pi\pi\pi\pi^0\nu_\tau$. 
These final states cover about $95\%$ of the total $\tau$ width, and have one (1-prong) or 
three (3-prong) charged particles, with the possible addition of a $\pi^0$. Since final states  
containing one or more $\pi^0$ cover about 40\% of the tau decay modes, an increase in the 
EMC coverage improves substantially the efficiency of tau identification. 

A large background arises from $B$-meson decays with undetected or misidentified particles, such 
as $B \rightarrow \pi^0 \ell \nu$ or $B \rightarrow \eta \ell \nu$. These backgrounds are further 
rejected using, $E_{extra}$, the total neutral energy in the detector of particles not associated 
with either $B$-meson. Signal events peak at low $E_{extra}$, while background events, which 
contain additional sources of neutral clusters, tend to be distributed at higher values. The 
discriminating power of this variables obviously increases with the calorimeter coverage. The 
signal and background levels are finally extracted by fitting the beam-energy substituted mass 
$m_{ES}=\sqrt{s/4-p_B^2}$ distribution of the tag $B$-mesons.

The performance of the backward EMC is assessed by comparing the signal-to-background ratio, $S/B$, 
and the statistical precision, $S/\sqrt{S+B}$, of the expected signal with and without the backward 
EMC. The addition of the backward EMC increases the signal-to-noise ratio by $\sim 18\%$ ($\sim ??\%$) 
and the statistical significance by $\sim 4\%$ ($\sim ??\%$) for hadronic (semileptonic) $B$-tagging. It 
is worth mentioning that the inclusive of the backward EMC not only improves the background rejection, 
but the $B$-tagging efficiency as well.


==> EMC/EMC-Barrel-cites.tex <==
\begin{thebibliography}{99}

%\cite{Zhu:1998eh}









\end{thebibliography}

\newpage




==> EMC/EMC-CostSchedule.tex <==
\tdrsec{Cost \& Schedule}

This will appear elsewhere.

\tdrsubsec{WBS structure}

\tdrsubsec{Gantt chart}

\tdrsubsec{Basis of estimates}

\tdrsubsec{Cost and schedule risks}



==> EMC/EMC-Trigger.tex <==
\tdrsec{Trigger}

This is a reminder that we need a synopsis of the EMC trigger somewhere
in the EMC chapter, although the detailed description will be in the ETD chapter.
It is to be determined whether this should be in a separate section or merged with
the three sub-calorimeter sections.

\tdrsubsec{Calorimeter readout trigger}
\tdrsubsubsec{Normal mode}
\tdrsubsubsec{Calibration mode}
\tdrsubsec{Calorimeter trigger primitives}



==> EMC/EMC-WhitePaper.tex <==
\begin{center}
{\bf White Paper text follows, for reference:}
\end{center}

\vskip.5cm

%This is the EMC section (5-6 pages)

% EMC chapter for 2009/10 white paper

The \superb\ electromagnetic calorimeter (EMC) provides energy
and direction measurement of photons and electrons, and is an
important component in the identification of electrons versus
other charged particles.
The system contains three components, shown in Figure~\ref{fig:det:superb}:
the barrel calorimeter, reused from \babar;
the forward endcap calorimeter, replacing the \babar\ forward endcap;
and the backward endcap calorimeter, a new device improving the
backward solid angle coverage.
Table~\ref{tab:SolidAngle} details the solid angle coverage of each
calorimeter. The total solid angle covered for a massless particle in the center-of-mass (CM)
is 94.1\% of 4$\pi$.


In addition to the \babar\ simulation for the barrel
calorimeter, simulation packages for the new forward and backward endcaps have
been developed, both in the form of a full simulation using the Geant4
toolkit and in the form of a fast simulation package for parametric
studies. These packages are used in the optimization of the calorimeter
and to study the physics impact of different options.

\tdrsec{Barrel Calorimeter}

The barrel calorimeter for \superb\ is the existing \babar\ CsI(Tl)
crystal calorimeter.\cite{bib:BaBarNIM1} Estimated rates and
radiation levels indicate that this system will continue
to survive and function in the \superb\ environment.
It covers $2\pi$ in azimuth
and polar angles from 26.8\degrees to 141.8\degrees in the lab.
There are 48 rings of crystals in polar angle, with 120 crystals in each azimuthal ring, for
a total of 5,760 crystals. The crystal length ranges from $16\Xrad$ to $17.5\Xrad$.
They are readout by two redundant PIN diodes connected to a multi-range amplifier.
A source calibration system allows calibrating the calorimeter with 6.13\mev photons from
the $^{16}N$ decay chain.
The \babar\ barrel calorimeter will be largely unchanged
for \superb; we indicate planned changes below.

Adding one more ring of crystals at the backward
end of the barrel is under consideration. These crystals would be obtained from the current \babar\ forward calorimeter, that will not be reused in \superb. Space is already available for the
additional crystals in the existing mechanical structure, although some
modification would be required to accommodate the additional readout.

The existing barrel PIN diode readout is kept at \superb.
In order to accommodate the higher event rate, the shaping
time is decreased. The existing ``CARE'' chip~\cite{bib:CARE} covers the
required dynamic range by providing four
different gains to be digitized in a ten-bit ADC. However,
this system is old, and the failure rate of the analog-to-digital
boards (ADBs) is unacceptably high. Thus, a new ADB has been
designed, along with a new analog board, the Very Front End (VFE) board, shown
in Figure~\ref{fig:VFE}.
The new design incorporates a dual-gain amplifier, followed by a
twelve-bit ADC. In order to provide good least-count resolution on the 6\mev\
calibration source, an additional calibration range is provided on the ADB.
The existing PIN diodes, with their redundancy, are expected to
continue to perform satisfactorily. They are epoxied to the crystals and
changing them would be a difficult operation.
\begin{figure}[hbt]
\begin{center}
\includegraphics[width=0.9\columnwidth]{VFEboard.pdf}
\end{center}
\caption{Block diagram for the Very Front End board, for the barrel and
forward endcap signal readout.}
\label{fig:VFE}
\end{figure}

\tdrsec{Forward Endcap Calorimeter}

The forward electromagnetic calorimeter for \superb\ is a new
device replacing the \babar\ CsI(Tl) forward calorimeter, with coverage
starting at the end of the barrel and extending down
to 270\mrad ($\cos\theta=0.965$) in the laboratory.
Because of the increased background levels, a faster and more radiation hard
material, such as LYSO or pure CsI, is required in the forward calorimeter.
The baseline design is based on LYSO (Lutetium Yttrium Orthosilicate, with Cerium
doping) crystals. The advantages of LYSO include
a much shorter scintillation time constant (LYSO: 40\ns, CsI(Tl): 680\ns and 3.34\mus), a smaller Moli\`ere
radius (LYSO: 2.1\cm, CsI: 3.6\cm), and greater resistance to radiation damage. One radiation
length is 1.14\cm in LYSO and 1.86\cm in CsI. An alternative choice is pure
CsI~\cite{bib:BelleEMC}. However, the light output is much smaller, making
LYSO preferable.

There are 20 rings of crystals, arranged in four groups of 5 layers each.
The crystals maintain the almost projective geometry of the barrel.
Each group of five layers is arranged in modules five crystals wide.
The preferred endcap structure is a continuous ring. However,
the numbers of modules in each group layers are multiples of 6, allowing the
detector to be split in two halves, should that be necessary from
installation considerations. The grouping of crystals is summarized in Table~\ref{tab:LYSOlayout}
and illustrated in Figure~\ref{fig:fwdEMCxtals}.

\begin{table}[tbp]
\caption{Layout of the forward endcap calorimeter.}
\begin{center}
\begin{tabular}{ccc}
Group&Modules& Crystals\\
1&36&900\\
2&42&1050\\
3&48&1200\\
4&54&1050\\
Total && 4500
\end{tabular}
\end{center}
\label{tab:LYSOlayout}
\end{table}

\begin{figure}
\begin{center}
\includegraphics[width=3in]{fwdEMCxtals.pdf}
\end{center}
\caption{Arrangement of the LYSO crystals in groups of rings.}
\label{fig:fwdEMCxtals}
\end{figure}

Each crystal is up to $2.5\times 2.5\cma$ at the back end, with a
projective taper to the front. The maximum
transverse dimensions are dictated by the Moli\`ere radius and by the desire to obtain two crystals
from a boule. The length of each crystal is approximately 20\cm, or 17.5\Xrad.

\tdrsubsec{Mechanical Structure}
The support for the crystals is an alveolar structure (\ie, a sort of egg-crate structure, with a cell for each crystal) constructed of
either carbon fiber or glass fiber and bounded by two
conical structures at the radial extremes.
To minimize the dead material between the endcap and the barrel,
the outer cone is made of carbon fiber with a thickness between 6 and 10\mm.
The inner cone is instead made of 20 to 30\mm-thick aluminum.

With the inclusion of the source calibration system, described below, and the front
cooling system, the total front wall thickness may reach 20---30\mm. A good solution
that minimizes material in front of the calorimeter is to embed the
pipes  into the foam core of a sandwich panel completed by two
skins of 2---3\mm carbon fiber. A lighter alternative under investigation is
to use depressions in pressed aluminum sheets forming the two
skins of the front wall to form the calibration and
cooling circuits.
The support at the back, providing the load-bearing
support for the forward calorimeter, is constructed in stainless steel as either
an open frame or closed plate.

\tdrsubsec{Readout System}
Two possible readouts are under study: PIN diodes as used the barrel and
APDs (Avalanche Photodiodes). As for the barrel, redundancy is achieved with
2 APDs or PIN diodes per crystal. APDs, with a low-noise gain of order 50,
offer the possibility of measuring signals
from sub-\mev radioactive sources. This would obviate the need for a step
with photomultipliers during the uniformity measurement process during calorimeter
construction. A concern in the \superb\ environment is the nuclear counter effect
from background neutrons. APDs also have an advantage over PIN diodes here. Nevertheless,
it may be desirable to use the redundant photodetectors with a comparator arrangement
to eliminate spurious large signals due to this background. This is under
investigation.
The disadvantage of APDs is the gain dependence on temperature, which can be of order $2\%/^\circ C$ (e.g.~\cite{bib:CMSTDR}). This
requires tight control of the readout temperature.  The same electronics as
for the barrel is used, with an adjustment to the VFE board gain with the
APD choice.

\tdrsubsec{Calibration and Beam Test}
The source calibration system is a new version of the 6.13\mev calibration
system already used in \babar.
%, as also used for the barrel calorimeter.
This system uses a neutron generator to produce activated
$^{16}N$ from fluorine in Fluorinert~\cite{bib:Fluorinert} coolant. The activated coolant is circulated near the front
of the crystals in the detector, where the $^{16}N$ decays with a 7\sec half-life. The 6.13\mev photons are produced in the decay chain $^{16}N\to ^{16}O^* + \beta,\ ^{16}O^*\to ^{16}O + \gamma$.

Two beam tests are planned to study the LYSO performance and the readout
options. The first beam test is at Frascati's Beam Test Facility, covering
the 50---500\mev\ energy range. The second beam test is at CERN, to cover the
\gev\ energy range.
In addition, a prototype alveolar
support structure is being constructed for the beam test.

\tdrsubsec{Performance Studies}
Simulation studies are underway to optimize the detector
configuration. It is important to use a
realistic clustering algorithm in these studies, since in
actual events multiple particles can overlap, requiring clever pattern
recognition. Figure~\ref{fig:FwdCluster} shows how the measured energy
distribution changes for different reconstruction algorithms.


%\begin{figure*}
%\begin{center}
%\subfloat[Optical design of FDIRC (dimensions are in \cm).]{\includegraphics[width=0.4\textwidth]{FDIRC_design_a.pdf} }
%\subfloat[Its equivalent in the \geant4 MC model.]{\includegraphics[width=0.4\textwidth]{FDIRC_design_b.pdf}}
%\end{center}
%\caption{Forward DIRC Design.}
%\label{fig:FDIRC_design}
%\end{figure*}

\begin{figure*}
\begin{center}
\includegraphics[width=3.3in]{FwdClusterL.pdf}\includegraphics[width=3.3in]{FwdClusterR.pdf}
\end{center}
\caption{Effect on the measured energy distribution for
various reconstruction algorithms. The ``No clustering'' distribution
results from simply adding all crystal energies greater than 1\mev.
The ``Clustering'' distribution results from the algorithm used in
\babar. The curves labeled $5\times 5$ crystal matrix and $3\times 3$ crystal matrix are simple sums of energy deposits in 25 or 9 crystals, respectively, centered on the crystal with the most energy. Left: 100\mev photons; Right: 1\gev photons.
}
\label{fig:FwdCluster}
\end{figure*}

Particular attention has been devoted to the study of the effect of material in front of the forward
calorimeter, for instance due to a proposed forward PID device.
Material in front of the calorimeter enhances the low-energy tail of the measurement, although peak
width measures, such as the FWHM, are almost unaffected, as shown in Figure~\ref{fig:EmeasEbeam}.
for the cases of 25 and 60\mm of quartz in front of the calorimeter.

\begin{figure}
\begin{center}
\includegraphics[width=3.3in]{EmeasEbeam.pdf}
\end{center}
\caption{Ratio of the measured/beam energy in the forward calorimeter for 100\mev\
photons and two different thickness of quartz, as well as no quartz, in front
of the calorimeter.}
\label{fig:EmeasEbeam}
\end{figure}

A more meaningful measure that we may use is:
$$
 f_{90}\equiv {E_{\rm true} - E_{90}\over E_{\rm true}},
$$
where $E_{\rm true}$ is the energy of the generated photon and $E_{90}$ gives
the 90\% quantile of the measured energy distribution,
\ie, 90\% of measurements of the photon energy are above this value.
Figure~\ref{fig:FwdMatRes} shows the effect on
the $f_{90}$ measure of resolution as a function of the quartz thickness.

\begin{figure}
\begin{center}
\includegraphics[width=3.3in]{FwdMatRes.pdf}
\end{center}
\caption{The effect of quartz material in front of the forward calorimeter, as a function of thickness and photon energy. The ordinate is $f_{90}$, explained in the text, expressed as per cent.}
\label{fig:FwdMatRes}
\end{figure}

Ideally, the transition between the barrel and forward calorimeters should be smooth, in
order to contain the electromagnetic showers and to keep pattern recognition simple.
Some possibilities for particle identification however require the forward calorimeter to
be moved back from the IP relative to the smooth transition point. The effect of this
on photon energy resolution has been studied, see Figure~\ref{fig:FWzStudy}. The resolution
degrades in the barrel-endcap transition region as expected, but there is substantially
no dependence on the z-position.

\begin{figure*}
\begin{center}
\includegraphics[width=3.in]{FWzCenter.pdf}\hskip1cm\includegraphics[width=3.in]{FWzTransition.pdf}
\end{center}
\caption{Effect on resolution of z-position of forward calorimeter.
Left: Resolution as a function of position for showers away from the
edges of the forward calorimeter.
Right: Resolution as a function of position for showers in the
transition region between the barrel and forward calorimeters. Note the different scales.
}
\label{fig:FWzStudy}
\end{figure*}

\tdrsec{Backward Endcap Calorimeter}

The backward electromagnetic calorimeter for \superb\ is a new device with the principal
intent of improving hermeticity at modest cost. Excellent energy
resolution is not a requirement, since there is significant material
from the drift chamber in front of it. Thus a high
quality crystal calorimeter is not planned for the backward region.
The proposed device is based on a multi-layer lead-scintillator stack with
longitudinal segmentation providing capability for $\pi/e$ separation.



The backward calorimeter is located starting at z$=-1320\mm$, allowing room for
the drift chamber front end electronics.  The inner radius is 310\mm, and the outer
radius 750\mm. The total thickness is 12\Xrad. It is constructed from a sandwich of
2.8\mm Pb alternating with 3\mm plastic scintillator (\eg, BC-404 or BC-408). The scintillator light
is collected for readout in wavelength-shifting fibers (\eg, 1\mm Y11).

To provide for transverse spatial
shower measurement, each layer of scintillator is segmented into strips. The segmentation
alternates among three different patterns for different layers:
\begin{itemize}
\item Right-handed logarithmic spiral;
\item Left-handed logarithmic spiral; and
\item Radial wedge.
\end{itemize}
This set of patterns is repeated eight times to make a total
of 24 layers.
With this arrangement, the fibers all emerge at the outer radius of the
detector. There are 48 strips per layer, for a total of 1152 strips.
The strip geometry is illustrated in Figure~\ref{fig:backEMCgeom}


\begin{figure}
\begin{center}
\includegraphics[width=3in]{backEMCgeom.pdf}
\end{center}
\caption{The backward EMC, showing the scintillator strip
geometry for pattern recognition.}
\label{fig:backEMCgeom}
\end{figure}

It is desirable to maintain mechanical integrity by constructing the
scintillator layers with several strips from a single piece of scintillator,
and not completely severing them. Isolation is achieved by cutting grooves
at the strip boundaries. The optimization of this with respect
to cross-talk and mechanical properties is under investigation.

The readout fibers are embedded in grooves cut into the
scintillator. Each fiber is read out at the outer radius with a $1\times 1\mma$
multi-pixel photon counter (MPPC, or SiPM, for ``silicon photomultiplier'')~\cite{bib:MPPC}. A mirror
is glued to each fiber at the inner radius to maximize light collection.
The SPIROC (SiPM Integrated Read-Out Chip) integrated circuit~\cite{bib:SPIROC}
developed for the ILC is used to digitize the MPPC signals,
providing both TDC (100\ps) and ADC (12 bit) capability. Each chip contains 36 channels.

A concern with the MPPCs is radiation hardness. Degradation in performance
is observed in studies performed for the \superb\ IFR, beginning at
integrated doses of order $10^8$ 1-\mev-equivalent neutrons/\cma~\cite{bib:Faccini}.
%by T.~Takeshita for CALICE at a dose of $3\times 10^9$ neutrons/cm$^2$.
This needs to be studied further, and possibly mitigated with shielding.


\begin{figure*}
\begin{center}
\includegraphics[width=3.3in]{BwdSBleft.pdf}\includegraphics[width=3.3in]{BwdSBright.pdf}
\end{center}
\caption{Left: Signal-to-background ratio with and without
a backward calorimeter, as a function of the $E_{\rm extra}$ selection.
Right: Ratio of the S/B ratio with
a backward calorimeter to the S/B ratio without a
backward calorimeter, as a function of the $E_{\rm extra}$ selection.
}
\label{fig:BwdSB}
\end{figure*}

Simulation studies are being performed to investigate the performance gain  achieved by
the addition of the backward calorimeter. The $B\to\tau\nu_\tau$ decay presents an important physics channel where hermeticity
is a significant consideration. The measurement of the branching fraction has been studied in simulations to evaluate the effect
of the backward calorimeter. Events in which one $B$ decays to $D^0\pi$, with $D^0\to K^-\pi^+$, are used to tag the events,
%NOT DCS!  K^\pm\pi^\mp$, are used to tag the events,
and several of the highest branching fraction one-prong $\tau$ decays are used.

Besides the selection of the tagging $B$ decay, and one additional track for the $\tau$, the key selection criterion is on
$E_{\rm extra}$, the energy sum of all remaining clusters in the
EMC. This quantity is used to discriminate against
backgrounds by requiring events to have low values; a reasonable
criterion is to accept events with $E_{\rm extra} < 400\mev$.

%\begin{figure}
%\begin{center}
%\includegraphics[width=3.3in]{BwdSB.pdf}
%\end{center}
%\caption{%Backward calorimeter study for $B\to\tau\nu$ decays.
%Top: Signal-to-background ratio with and without
%a backward calorimeter, as a function of the $E_{\rm extra}$ selection.
%Bottom: Ratio of the $S/B$ ratio with
%a backward calorimeter to the $S/B$ ratio without a
%backward calorimeter, as a function of the $E_{\rm extra}$ selection.}
%\label{fig:BwdSB}
%\end{figure}

In this study we find that the signal-to-background ratio
is improved by approximately 20\% if the backward calorimeter
is present (Figure~\ref{fig:BwdSB}). The corresponding improvement
in precision (${\rm S}/\sqrt{{\rm S}+{\rm B}}$) for 75\invab is approximately 8\% (Figure~\ref{fig:bwdEMC_btotaunu}).
We note that only one tag mode has so far been investigated, and this study
is ongoing with work on additional modes to obtain results for a
more complete sample analysis. Also, the effect of background events
superimposed on the physics event has not been fully studied.

%\begin{figure}
%\begin{center}
%\includegraphics[width=3.3in]{BwdSSB.pdf}
%\end{center}
%\caption{%Backward calorimeter study for $B\to\tau\nu$ decays, for
%75 \invab.
%Top: Precision (${\rm S}/\sqrt{{\rm S}+{\rm B}}$) with and without
%a backward calorimeter, as a function of the $E_{\rm extra}$ selection.
%Bottom: Ratio of the precision with
%a backward calorimeter to the precision without a
%backward calorimeter, as a function of the $E_{\rm extra}$ selection. }
%\label{fig:BwdSSB}
%\end{figure}

%\begin{figure*}
%\begin{center}
%\includegraphics[width=3.3in]{BwdSSBleft.pdf}\includegraphics[width=3.3in]{BwdSSBright.pdf}
%\end{center}
%\caption{Backward calorimeter study for $B\to\tau\nu$ decays, for
%75 \invab.
%Left: Precision (${\rm S}/\sqrt{{\rm S}+{\rm B}}$) with and without
%a backward calorimeter, as a function of the $E_{\rm extra}$ selection.
%Right: Ratio of the precision with
%a backward calorimeter to the precision without a
%backward calorimeter, as a function of the $E_{\rm extra}$ selection.
%}
%\label{fig:BwdSSB}
%\end{figure*}

The possibility of using the backward endcap for
particle identification as a time-of-flight measuring device is also under investigation.
Figure~\ref{fig:BwdPID} shows, for example, for 100\ps timing
resolution, a separation of more than three standard deviations ($\sigma$) can
be achieved for momenta up to 1\gevc and approximately 1.5$\sigma$ up
to 1.5\gevc.

\begin{figure}
\begin{center}
\includegraphics[width=3.3in]{BwdPID.pdf}
\end{center}
\caption{Kaon-pion separation versus measured momentum for different
timing resolutions in the backward EMC region. The finite separation
for perfect timing resolution is because measured momentum is used.}
\label{fig:BwdPID}
\end{figure}


\tdrsec{R\&D}

\tdrsubsec{Barrel Calorimeter}

The main R\&D question for the barrel concerns the
shaping time. Simulation work is underway to
investigate  pile-up effects from backgrounds. In addition,
electronics and software issues connected with the
possibility of adding one more ring of CsI
crystals at the back end are still to be addressed.

\tdrsubsec{Forward Calorimeter}

The forward calorimeter is a new device, and we are
planning for two beam tests are planned to test the performance of
an LYSO crystal array as well as the
solutions for the
electronics and mechanical designs. The beam tests will also investigate the
use of PIN diodes and APDs as readout options as well as
the effect of material in front of the crystals in the beam test.
Simulation work is ongoing to predict performance and backgrounds.
Possible modifications to the electronics design to deal with
neutron nuclear-counter signals in the photodetector will be investigated.
There is an ongoing R\&D effort with vendors to produce crystals with
good light output and uniformity at an acceptable cost.
The crystal support and integration of the calibration and cooling
circuits with the mechanical structure is under investigation in
consultation with vendors.

\tdrsubsec{Backward Calorimeter}

A beam test of the backward calorimeter is also planned, probably concurrent
with the forward calorimeter beam test at CERN. The mechanical support and
segmentation of the plastic scintillator is being investigated for a
solution that achieves simplicity and acceptable cross-talk. The use of
multi-pixel photon counters is being studied, including the
radiation damage issue. The timing resolution for a possible time-of-flight
measurement is an interesting question. Further simulation studies are being made to
characterize the performance impact of the backward calorimeter.

%\vskip-8mm
\begin{thebibliography}{99}

\bibitem{bib:BaBarNIM1}
 B.~Aubert {\it et al.} (\babar\ Collaboration), {\it The \babar\ Detector}, \nima{479}, 1 (2002)
  [arXiv:hep-ex/0105044].
%Nucl. Instr. Meth, in Phys Res. {\bf A479} (2002) 1.

\bibitem{bib:CARE}
G.~Haller and D.~Freytag, IEEE Trans.\ Nucl.\ Sci. {\bf 43}, 1610 (1996).
% 1610.

\bibitem{bib:BelleEMC}
I.~Nakamura, {\it Belle Electromagnetic Calorimeter and its sBelle Upgrade},
J.\ Phys.\ Conf.\ Ser.\ {\bf 169}, 012003 (2009).

\bibitem{bib:CMSTDR}
CMS ECAL Technical Design Report, CERN/LHCC 97-33 (1997),
{\url{http://cms-ecal.web.cern.ch/cms-ecal/ECAL\_TDR/ref/C4\_P107-116.pdf}}.

\bibitem{bib:Fluorinert} Fluorinert is the trademark name for
polychlorotrifluoro-ethylene), manufactured by 3M Corporation,
St. Paul, MN, USA.

\bibitem{bib:MPPC} Hamamatsu S10362-11 series MPPC, {\url{http://jp.hamamatsu.com/resources/products/ssd/pdf/s10362-11series\_kapd1022e05.pdf}}.

\bibitem{bib:SPIROC} M.~Bouchel, {\it et al.}, {\it SPIROC (SiPM Integrated
Read-Out Chip): Dedicated very front-end electronics for an ILC prototype hadronic calorimeter with SiPM read-out}, NSS '07 IEEE {\bf 3}, 1857 (2007).

%% NEXT IS SAME as in IFR.tex
\bibitem{bib:Faccini}
M. Angelone {\it et al.}, {\it Silicon Photo-Multiplier radiation hardness tests with a beam controlled neutron source}, arXiv:1002.3480 [physics.ins-det].
\end{thebibliography}



==> ESH/ESH.tex <==
\tdrchap{Environmental Safety and Health}
WHO ?? Pages ??



==> ETD/ETD-org.tex <==
% Organizational Structure of Electronics, Trigger, DAQ and Online

{\color{blue} DB + UM + SL}

%The system has been designed with a very tight integration of hardware
%and software. Based on this and the experience when building and
%upgrading the \babar\ data acquisition and online systems, we propose
%that the organizational structure of ETD/Online



==> MDI/quick_demounting.tex <==
\tdrsec{ Quick demounting.
 \hfill {\color{green} M.Sullivan, F.Bosi, E.Paoloni - \color{red} 4 pages}}


==> MDI/synchrotron_radiation.tex <==
\tdrsec{ Synchrotron radiation background.
 \hfill {\color{green} M.Sullivan  - \color{red} 2 pages}}
\label{sec:mdi_syncrad}

In which
\begin{itemize}
\item the synchrotron radiation process is described
\item the simulation tools are presented
\item the shielding system is sketched
\item the losses at the beam pipe are reported
\item the dosed in the SVT are evaluated
\end{itemize}


==> PID/PID-Performance.tex <==
\tdrsec{ Projected FDIRC Performance  }

\tdrsubsec{ Reconstruction 
{ \color{green} Arnaud, Roberts } }

\tdrsubsec{ MC Simulation }
						
\tdrparagraph{ Fast simulation 
{ \color{green} Arnaud } }

\tdrparagraph{ Full simulation 
{ \color{green} Roberts } }

\tdrsubsec { Effect of Background on performance 
{ \color{green} Roberts } }
\label{sec:PID_FDIRC_Bkg_performance}



==> Physics/BDecays-tab.tex <==
\begin{center}
\begin{tiny}
%% B decays
\begin{tabular}{| l ||@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|} \hline
 & $J^{PC}$ &  $J/\psi\pi\pi$ &  $J/\psi\omega$ &  $J/\psi\gamma$ &  $J/\psi\phi$ &  $J/\psi\eta$ & $\psi(\rm{2S})\pi\pi$ & $\psi(\rm{2S})\omega$ & $\psi({\rm 2S})\gamma$ & $\chi_c\gamma$ & pp & $\Lambda\Lambda$ & $\Lambda_c\Lambda_c$ & $DD$ &$ DD^*$ & $D^*D^*$ & $D_s^{(*)}D_s^{(*)}$ & $\gamma\gamma$\\\hline\hline
X(3872) & $1^{++} $&{\green\bf S}&{ \green\bf S}&{ \green\bf S}& N/A & { \red\bf N/S} & N/A & N/A &{ \green\bf S}& { \red\bf N/S} & { \cyan\bf M/F} & { \cyan\bf M/F} & N/A & N/A &{ \green\bf S}& N/A & N/A & { \red\bf N/S}\\ 
& $2^{-+}$ &&&&&&&&&&&&&&&&&\\ \hline
X(3940) & JP+& { \cyan\bf M/F} &{ \green\bf S}& { \red\bf N/S} & N/A & N/A & N/A & N/A & { \cyan\bf M/F} & N/A & { \cyan\bf M/F} & { \cyan\bf M/F} & N/A & { \cyan\bf M/F} & { \red\bf N/S} & N/A &{\cyan \bf N}&{\cyan \bf N}\\ \hline
Z(3940) & 2++ & { \cyan\bf M/F} & { \cyan\bf M/F} & { \red\bf N/S} & N/A & N/A & N/A & N/A & { \cyan\bf M/F} & N/A & { \cyan\bf M/F} & { \cyan\bf M/F} & N/A & { \cyan\bf M/F} & { \cyan\bf M/F} & N/A &{\cyan \bf N}&{\cyan \bf N}\\ \hline
Y(4140) & JP+ & { \cyan\bf M/F} & { \cyan\bf M/F} &{\cyan \bf N}&{ \green\bf S}& N/A &{\cyan \bf N}& N/A &{\cyan \bf N}& N/A & { \cyan\bf M/F} & { \cyan\bf M/F} & N/A & { \cyan\bf M/F} &{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}\\ \hline
X(4160) & 0P+ & { \cyan\bf M/F} & { \cyan\bf M/F} &{\cyan \bf N}& { \cyan\bf M/F} & N/A &{\cyan \bf N}& N/A &{\cyan \bf N}& N/A & { \cyan\bf M/F} & { \cyan\bf M/F} & N/A & { \cyan\bf M/F} &{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}\\ \hline
Y(4260) & 1-- &{ \green\bf S}& N/A & N/A & N/A & { \cyan\bf M/F} &{\cyan \bf N}& N/A & N/A &{\cyan \bf N}& { \cyan\bf M/F} & { \cyan\bf M/F} & N/A &{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}& N/A\\ \hline
X(4350) & JP+ & { \cyan\bf M/F} & { \cyan\bf M/F} &{\cyan \bf N}& { \cyan\bf M/F} & N/A &{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}& N/A & { \cyan\bf M/F} & { \cyan\bf M/F} & N/A &{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}\\ \hline
Y(4350) & 1-- & { \cyan\bf M/F} & N/A & N/A & N/A & { \cyan\bf M/F} &{\cyan \bf N}& N/A & N/A &{\cyan \bf N}& { \cyan\bf M/F} & { \cyan\bf M/F} & N/A &{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}& N/A\\ \hline
Y(4660) & 1-- &{\cyan \bf N}& N/A & N/A & N/A  & { \cyan\bf M/F} &{\cyan \bf N}& N/A & N/A &{\cyan \bf N}& { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F} &{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}& N/A\\ \hline
\end{tabular}
\end{tiny}

\end{center}



==> Physics/GamGam-tab.tex <==
\begin{center}
\begin{tiny}
%% B decays
\begin{tabular}{| l ||@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|} \hline
 & $J^{PC}$ &  $J/\psi\pi\pi$ &  $J/\psi\omega$ &  $J/\psi\gamma$ &  $J/\psi\phi$ & $\psi(\rm{2S})\pi\pi$ & $\psi(\rm{2S})\omega$ & $\psi({\rm 2S})\gamma$ & $\chi_c\gamma$ & pp & $\Lambda\Lambda$ & $\Lambda_c\Lambda_c$ & $DD$ &$ DD^*$ & $D^*D^*$ & $D_s^{(*)}D_s^{(*)}$\\\hline\hline
X(3872) &$ 1^{++}$ [$2^{-+}$] &{\cyan \bf N}& N/F & N/F & N/A & N/A & N/A & N/F & {\cyan \bf M/F} & {\cyan \bf M/F} & N/A & {\cyan \bf M/F} &{\cyan \bf N}& N/A & N/A\\\hline
"X & Y (3940)" & $0^{-+}$ [$J^{P+}$] &{\cyan \bf N}&{\green \bf S}& N/F & N/A & N/A & N/A & N/F & {\cyan \bf M/F} & {\cyan \bf M/F} & N/A & {\green \bf S} &{\cyan \bf N}& N/A & N\\\hline
Z(3940) & $2^{++}$ &{\cyan \bf N}&{\green \bf S}   & N/F & N/A & N/A & N/A & N/F & {\cyan \bf M/F} & {\cyan \bf M/F} & N/A &{\green \bf S}&{\cyan \bf N}& N/A & N\\\hline
Y(4140) & $J^{P+}$ &{\cyan \bf N}& {\cyan \bf M/F} & N/F &{\red \bf N/S}&{\cyan \bf N}& N/A & N/F &{\cyan \bf N}&{\cyan \bf N}& N/A & {\cyan \bf M/F} &{\cyan \bf N}&{\cyan \bf N}& N\\\hline
X(4160) & $0^{P+}$ &{\cyan \bf N}& {\cyan \bf M/F} & N/F &{\red \bf N/S}&{\cyan \bf N}& N/A & N/F &{\cyan \bf N}&{\cyan \bf N}& N/A & {\cyan \bf M/F} &{\cyan \bf N}&{\cyan \bf N}& N\\\hline
X(4350) & $J^{P+}$ &{\cyan \bf N}&{\cyan \bf N}& N/F &{\green \bf S}&{\cyan \bf N}&{\cyan \bf N}& N/F &{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}&{\cyan \bf N}& N\\\hline
\end{tabular}
\end{tiny}

\end{center}


==> Physics/ISR-tab.tex <==
\begin{center}
\begin{tiny}
%% ISR
\begin{tabular}{| l ||@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|} \hline

&$J^{PC}$ &  $J/\psi\pi\pi$ &   $\psi(\rm{2S})\pi\pi$ & $J\psi\eta$ &  $\chi_c\gamma$ & pp & $\Lambda\Lambda$ & $\Lambda_c\Lambda_c$ & $DD$ &$ DD^*$ & $D^*D^*$ & $D_s^{(*)}D_s^{(*)}$ \\ \hline \hline
Y(4260) & $1^{--}$ & { \green \bf S}&  { \red\bf N/S} &  { \red\bf N/S} &  { \red\bf N/S} &  { \red\bf N/S} & { \cyan\bf M/F} & N/A &  { \red\bf N/S} &  { \red\bf N/S} &  { \red\bf N/S} &  { \red\bf N/S}\\ \hline
Y(4350) & $1^{--}$ &  { \red\bf N/S} & { \green \bf S}& { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F} & N/A & { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F}\\ \hline
Y(4660) & $1^{--}$ &  { \red\bf N/S} & { \green \bf S}& { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F} & { \green \bf S}& { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F} & { \cyan\bf M/F}\\ \hline
\end{tabular}
\end{tiny}

\end{center}


==> Physics/Recoil-tab.tex <==
\begin{center}
\begin{tiny}
%% B decays
\begin{tabular}{| l ||@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|} \hline
 & $J^{PC}$ &  $J/\psi\pi\pi$ &  $J/\psi\omega$ &  $J/\psi\gamma$ &  $J/\psi\phi$ & $\psi(\rm{2S})\pi\pi$ & $\psi(\rm{2S})\omega$ & $\psi({\rm 2S})\gamma$ & $\chi_c\gamma$ & pp & $\Lambda\Lambda$ & $\Lambda_c\Lambda_c$ & $DD$ &$ DD^*$ & $D^*D^*$\\\hline\hline

X(3872) & $1^{++} $[$2^{-+}$] & N/F &{\cyan \bf N}& N/F & N/A & N/F & N/A & N/F & N/F & N/F & N/F & N/A &{ \cyan\bf M/F} &{ \cyan\bf M/F} & N/A\\\hline
"X & Y (3940)" & $0^{-+}$ [$J^{P+}$] & N/F &{\cyan \bf N}& N/F & N/A & N/F & N/A & N/F & N/F & N/F & N/F & N/A &{ \green\bf S} &{ \cyan\bf M/F} & N/A\\\hline
Z(3940) & $2^{++} $& N/F &{\cyan \bf N}& N/F & N/A & N/F & N/A & N/F & N/F & N/F & N/F & N/A &{ \cyan\bf M/F} &{ \cyan\bf M/F} & N/A\\\hline
Y(4140) & $J^{P+}$ & N/F &{\cyan \bf N}& N/F &{\cyan \bf N}& N/F & N/A & N/F & N/F & N/F & N/F & N/A &{ \cyan\bf M/F} &{ \cyan\bf M/F} &{ \cyan\bf M/F}\\\hline
X(4160) & $0^{P+} $& N/F &{\cyan \bf N}& N/F &{\cyan \bf N}& N/F & N/A & N/F & N/F & N/F & N/F & N/A &{ \cyan\bf M/F} &{ \green\bf S}&{ \cyan\bf M/F}\\\hline
X(4350) & $J^{P+}$ & N/F &{\cyan \bf N}& N/F &{\cyan \bf N}& N/F &{\cyan \bf N}& N/F & N/F & N/F & N/F & N/F &{ \cyan\bf M/F} &{ \cyan\bf M/F} &{ \cyan\bf M/F}\\\hline

\end{tabular}
\end{tiny}

\end{center}


==> SVT/svt_power_supply.tex <==
\tdrsubsec{Power Supply \hfill {\color{green}  - \color{red} 2}}

==> dtdrAccOverview.tex <==
%%
%% compile just AccOverview chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrAccOverview
%% bibtex AccOverview
%% pdflatex dtdrAccOverview
%% pdflatex dtdrAccOverview
%%
\newcommand{\inclCmds}{%
  \includeonly{AccOverview}
}
\input{dtdr.tex}


==> dtdrBudget.tex <==
%%
%% compile just Budget chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrBudget
%% bibtex Budget
%% pdflatex dtdrBudget
%% pdflatex dtdrBudget
%%
\newcommand{\inclCmds}{%
  \includeonly{Budget}
}
\input{dtdr.tex}


==> dtdrComp.tex <==
%%
%% compile just COMP chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrComp
%% bibtex COMP
%% pdflatex dtdrComp
%% pdflatex dtdrComp
%%
\newcommand{\inclCmds}{%
  \includeonly{COMP}
}
\input{dtdr.tex}


==> dtdrDch.tex <==
%%
%% compile just DCH chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrDch
%% bibtex DCH
%% pdflatex dtdrDch
%% pdflatex dtdrDch
%%
\newcommand{\inclCmds}{%
  \includeonly{DCH}
}
\input{dtdr.tex}


==> dtdrDetOverview.tex <==
%%
%% compile just DetOverview chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrDetOverview
%% bibtex DetOverview
%% pdflatex dtdrDetOverview
%% pdflatex dtdrDetOverview
%%
\newcommand{\inclCmds}{%
  \includeonly{DetOverview}
}
\input{dtdr.tex}


==> dtdrElex.tex <==
%%
%% compile just ELEX chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrElex
%% bibtex ELEX
%% pdflatex dtdrElex
%% pdflatex dtdrElex
%%
\newcommand{\inclCmds}{%
  \includeonly{ELEX}
}
\input{dtdr.tex}


==> dtdrEmc.tex <==
%%
%% compile just EMC chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrEmc
%% bibtex EMC
%% pdflatex dtdrEmc
%% pdflatex dtdrEmc
%%
\newcommand{\inclCmds}{%
  \includeonly{EMC}
}
\input{dtdr.tex}


==> dtdrEsh.tex <==
%%
%% compile just ESH chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrEsh
%% bibtex ESH
%% pdflatex dtdrEsh
%% pdflatex dtdrEsh
%%
\newcommand{\inclCmds}{%
  \includeonly{ESH}
}
\input{dtdr.tex}


==> dtdrEtd.tex <==
%%
%% compile just ETD chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrEtd
%% bibtex ETD
%% pdflatex dtdrEtd
%% pdflatex dtdrEtd
%%
\newcommand{\inclCmds}{%
  \includeonly{ETD}
}
\input{dtdr.tex}


==> dtdrFrontmatter.tex <==
%%
%% compile just PID chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrPid
%% bibtex PID
%% pdflatex dtdrPid
%% pdflatex dtdrPid
%%
\newcommand{\inclCmds}{%
  \includeonly{frontmatter}
%  \includeonly{preface}  % Use input in subdirectories, not include
%  \includeonly{authors}
}
\input{dtdr.tex}


==> dtdrIfr.tex <==
%%
%% compile just IFR chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrIfr
%% bibtex IFR
%% pdflatex dtdrIfr
%% pdflatex dtdrIfr
%%
\newcommand{\inclCmds}{%
  \includeonly{IFR}
}
\input{dtdr.tex}


==> dtdrIntegration.tex <==
%%
%% compile just Integration chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrIntegration
%% bibtex Integration
%% pdflatex dtdrIntegration
%% pdflatex dtdrIntegration
%%
\newcommand{\inclCmds}{%
  \includeonly{Integration}
}
\input{dtdr.tex}


==> dtdrIntroduction.tex <==
%%
%% compile just Introduction chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrIntroduction
%% bibtex Introduction
%% pdflatex dtdrIntroduction
%% pdflatex dtdrIntroduction
%%
\newcommand{\inclCmds}{%
  \includeonly{Introduction}
}
\input{dtdr.tex}


==> dtdrMagnet.tex <==
%%
%% compile just Magnet chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrMagnet
%% bibtex Magnet
%% pdflatex dtdrMagnet
%% pdflatex dtdrMagnet
%%
\newcommand{\inclCmds}{%
  \includeonly{Magnet}
}
\input{dtdr.tex}


==> dtdrManagement.tex <==
%%
%% compile just Management chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrManagement
%% bibtex Management
%% pdflatex dtdrManagement
%% pdflatex dtdrManagement
%%
\newcommand{\inclCmds}{%
  \includeonly{Management}
}
\input{dtdr.tex}


==> dtdrMdi.tex <==
%%
%% compile just MDI chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrMdi
%% bibtex MDI
%% pdflatex dtdrMdi
%% pdflatex dtdrMdi
%%
\newcommand{\inclCmds}{%
  \includeonly{MDI}
}
\input{dtdr.tex}


==> dtdrPhysics.tex <==
%%
%% compile just Physics chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrPhysics
%% bibtex Physics
%% pdflatex dtdrPhysics
%% pdflatex dtdrPhysics
%%
\newcommand{\inclCmds}{%
  \includeonly{Physics}
}
\input{dtdr.tex}


==> dtdrPid.tex <==
%%
%% compile just PID chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrPid
%% bibtex PID
%% pdflatex dtdrPid
%% pdflatex dtdrPid
%%
\newcommand{\inclCmds}{%
  \includeonly{PID}
}
\input{dtdr.tex}


==> dtdrSupport/babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   14/08/12 A. Bevan       Merge DTDR version with physics macros for ESG 2012 
%%%%%   Revised   01/28/10 F.Forti - added \ie and \eg
%%%%%	Revised   01/04/10 S. Luitz - cleaned up data size and rate macros
%%%%%	Revised   01/04/10 S. Luitz for SuperB: corrected \gbsps macro
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

\RequirePackage{hyperref}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar {\texorpdfstring{{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}\xspace}{BaBar}}

%%%%%%%%%%%%%%%%%%%% SUPERB

%\def\superb   {\texorpdfstring{{Super$\!\!\;B$\xspace}}{SuperB\xspace}}
\def\superb {\texorpdfstring{{Super\kern-0.04em\emph{B}}\xspace}{SuperB\xspace}}
\def\SuperB   {\superb}

%%%%%%%%%%%%%%%%%%%% OTHER EXPERIMENTS

\def\sff{Super Flavour Factory\xspace}
\def\sffs{Super Flavour Factories\xspace}
\def\lhcb {LHCb\xspace}
\def\besthree {BES III\xspace}
\def\lhc {LHC\xspace}
\def\slhc {SLHC\xspace}
\def\atlas {ATLAS\xspace}
\def\CMS {CMS\xspace}
\def\meg {MEG\xspace}
\def\koto {KOTO\xspace}
\def\comet {COMET\xspace}
\def\mutoe {Mu2e\xspace}
\def\belle {Belle\xspace}
\def\belletwo {Belle II\xspace}

\def\fastsim {FastSim\xspace}

\def\dgwg{Detector Geometry Working Group\xspace}
\def\tof{time-of-flight\xspace}
\def\ftof{DIRC-like forward time-of-flight detector\xspace} % Name to be updated

%% Added from Valencia files

\def\tauhhp{\ensuremath{\tau_{hh}^+}}
\def\tauhhm{\ensuremath{\tau_{hh}^-}}
\def\tauhh{\ensuremath{\tau_{hh}}}
\def\tauKpi{\ensuremath{\tau_{K\pi}}}
\def\yCP{\ensuremath{y_{C\!P}}}
\def\deltaY{\ensuremath{\Delta Y}}

\def\DZ{\ensuremath{{D}^{\rm{0}}}}
\def\DZB{\ensuremath{\overline{{D}}^{\rm{0}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace}
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\D       {\ensuremath{D}\xspace}
%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace}
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
%\def\Y#1S{}% no space before {...}!
%\def\OneS  {\Y1S}
%\def\TwoS  {\Y2S}
%\def\ThreeS {\Y3S}
%\def\FourS {\Y4S}
%\def\FiveS {\Y5S}
\def\OneS {\ensuremath{\Upsilon{(1S)}}\xspace}
\def\TwoS {\ensuremath{\Upsilon{(2S)}}\xspace}
\def\ThreeS {\ensuremath{\Upsilon{(3S)}}\xspace}
\def\FourS {\ensuremath{\Upsilon{(4S)}}\xspace}
\def\FiveS {\ensuremath{\Upsilon{(5S)}}\xspace}
\def\NS {\ensuremath{\Upsilon{(nS)}}\xspace}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar {\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar {\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar {\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar {\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar {\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar {\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb {\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}

\newcommand{\taumg}      {\ensuremath{\tau^{\pm} \to \mu^{\pm} \gamma}\xspace}
\newcommand{\taueg}      {\ensuremath{\tau^{\pm} \to e^{\pm} \gamma}\xspace}
\newcommand{\taulg}      {\ensuremath{\tau^{\pm} \to \ell^{\pm} \gamma}\xspace}
\newcommand{\taueee}      {\ensuremath{\tau^{\pm} \rightarrow e^{\pm}e^+e^-}\xspace }
\def\taummm      {\ensuremath{\tau^{\pm} \rightarrow \mu^{\pm}\mu^+\mu^-}\xspace }
\def\tauemm      {\ensuremath{\tau^{\pm} \rightarrow e^{\pm}\mu^+\mu^-}\xspace }
\def\taumee      {\ensuremath{\tau^{\pm} \rightarrow \mu^{\pm}e^+e^-}\xspace}
\def\taulh       {\ensuremath{\tau^{\pm} \rightarrow \ell^{\pm}h^0}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}}
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}}
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}}
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}}
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}}
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}}
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}}
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}}
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}}
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}}
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\msquare {\ensuremath{{\rm \,m}^2}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\cubicm   {\ensuremath{{\rm \,m}^3}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}
\def\designlumi {\ensuremath{10^{36}\cms}\xspace}
\def\lumi {\cms\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}

%Mass
\def\gm   {\ensuremath{\rm \,g}\xspace}
\def\kg   {\ensuremath{\rm \,kg}\xspace}
\def\ton  {\ensuremath{{\rm \,t}}\xspace}

\def\gmps {\ensuremath{\rm \,g/s}\xspace} 


%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\eg{\ensuremath {e.g.}}
\def\ie{\ensuremath {i.e.}}

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\pct {\ensuremath{{\rm \,\%}}\xspace}





%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}

\def\muF  {\ensuremath{\,\mu{\rm F}}\xspace}
\def\muH  {\ensuremath{\,\mu{\rm H}}\xspace}
\def\nF   {\ensuremath{\rm \,nF}\xspace}
\def\nH   {\ensuremath{\rm \,nH}\xspace}
\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm \,K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}

%\renewcommand{\bar}[1]{\overline{#1}}

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\BFs{$B$ Factories}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\btolnu     {\ensuremath{B^\pm\to \ell^\pm \nu}}
\def\btoenu     {\ensuremath{B^\pm\to e^\pm \nu}}
\def\btomunu     {\ensuremath{B^\pm\to \mu^\pm \nu}}
\def\btotaunu     {\ensuremath{B^\pm\to \tau^\pm \nu}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing

\def\bit	{\ensuremath{{\rm \,bit}}\xspace}
\def\kbit	{\ensuremath{{\rm \,kbit}}\xspace}
\def\kbits	{\kbit} % no more plural of units - deprecated
\def\kbitps	{\ensuremath{{\rm \,kbit/s}}\xspace}
\def\kbitsps	{\kbitps} % no more plural of units - deprecated
\def\kbps	{\kbitps} % for compatibility - deprecated
\def\kbsps	{\kbitsps} % for compatibility - deprecated

\def\kbyte      {\ensuremath{{\rm \,kByte}}\xspace}
\def\kbytes	{\kbyte}
\def\kbyteps    {\ensuremath{{\rm \,kByte/s}}\xspace}
\def\kbytesps	{\kbyteps}


\def\mbyte	{\ensuremath{{\rm \,MByte}}\xspace}
\def\mbytes	{\mbyte}
\def\mbyteps	{\ensuremath{{\rm \,MByte/s}}\xspace}
\def\mbytesps	{\mbyteps}

\def\mbit	{\ensuremath{{\rm \,Mbit}}\xspace}
\def\mbits	{\mbit}
\def\mbitps	{\ensuremath{{\rm \,Mbit/s}}\xspace}
\def\mbitsps	{\mbitps}
\def\mbps	{\mbitps} % for compatibility - deprecated
\def\mbsps	{\mbitsps} % for compatibility - deprecated

\def\gbit	{\ensuremath{{\rm \,Gbit}}\xspace}
\def\gbits	{\gbit}
\def\gbitps	{\ensuremath{{\rm \,Gbit/s}}\xspace}
\def\gbitsps	{\gbitps}
\def\gbps	{\gbitps} % for compatibility - deprecated
\def\gbsps	{\gbitsps} % for compatibility - deprecated


\def\gbyte	{\ensuremath{{\rm \,GByte}}\xspace}
\def\gbytes	{\gbyte}
\def\gbyteps	{\ensuremath{{\rm \,GByte/s}}\xspace}
\def\gbytesps	{\gbyteps}

\def\tbyte	{\ensuremath{{\rm \,TByte}}\xspace}
\def\tbytes	{\tbyte}
\def\tbyteps	{\ensuremath{{\rm \,TByte/s}}\xspace}
\def\tbytesps	{\tbyteps}
\def\tbyteph	{\ensuremath{{\rm \,TByte/h}}\xspace}
\def\tbytesph   {\tbyteph}
\def\tbytepd	{\ensuremath{{\rm \,TByte/day}}\xspace}
\def\tbytespd   {\tbytepd}

\def\pbyte	{\ensuremath{{\rm \,PByte}}\xspace}
\def\pbytepy    {\ensuremath{{\rm \,PByte/yr}}\xspace}

\def\tbpy       {\ensuremath{{\rm \,TByte/yr}}\xspace}

\def\khs        {\ensuremath{{\rm \,kHS06}}\xspace}
\def\mhs	{\ensuremath{{\rm \,MHS06}}\xspace}

\def\tbpab	{\ensuremath{\tbyte/\invab}}
\def\khspab	{\ensuremath{\khs/\invab}}


%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{\ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps  {\ensuremath{\varepsilon}\xspace}
\def\epsK {\ensuremath{\varepsilon_K}\xspace}
\def\epsB {\ensuremath{\varepsilon_B}\xspace}
\def\epsp {\ensuremath{\varepsilon^\prime_K}\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
\def\CPV               {\ensuremath{C\!P} violation\xspace}
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}},
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|,
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

% magnitudes
\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

% complex elements
\def\vud  {\ensuremath{V_{ud}}\xspace}
\def\vcd  {\ensuremath{V_{cd}}\xspace}
\def\vtd  {\ensuremath{V_{td}}\xspace}
\def\vus  {\ensuremath{V_{us}}\xspace}
\def\vcs  {\ensuremath{V_{cs}}\xspace}
\def\vts  {\ensuremath{V_{ts}}\xspace}
\def\vub  {\ensuremath{V_{ub}}\xspace}
\def\vcb  {\ensuremath{V_{cb}}\xspace}
\def\vtb  {\ensuremath{V_{tb}}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}




% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
% update the following based on input from John Ripka, Asst. Editor at PRL, August 2006
\newcommand{\nimBaseA}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}}
% add commands for NIM articles from earlier periods
% for NIM articles from 1981-1983
\newcommand{\oldnim}    [1]  {Nucl.\ Instrum.\ Methods Phys.\ Res.~{\bf #1}}
% for NIM articles prior to 1981
\newcommand{\oldernim}  [1]  {Nucl.\ Instrum.\ Methods~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
%\def\geantFour  {\mbox{\tt GEANT4}\xspace}
\def\geantFour  {\mbox{\sc Geant4}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}


==> dtdrSvt.tex <==
%%
%% compile just SVT chapter of TDR
%%
%% please compile as follows:
%%
%% pdflatex dtdrSvt
%% bibtex SVT
%% pdflatex dtdrSvt
%% pdflatex dtdrSvt
%%
\newcommand{\inclCmds}{%
  \includeonly{SVT}
}
\input{dtdr.tex}

